Can Atomic Step Decomposition Enhance the Self-structured Reasoning of Multimodal Large Models?

In this paper, we address the challenging task of multimodal mathematical reasoning by incorporating the ability of "slow thinking" into multimodal large language models (MLLMs). Our core idea is that different levels of reasoning abilities can be combined dynamically to tackle questions with different complexity. To this end, we propose a paradigm of Self-structured Chain of Thought (SCoT), which is composed of minimal semantic atomic steps. Different from existing methods that rely on structured templates or free-form paradigms, our method can not only generate cognitive CoT structures for various complex tasks but also mitigates the phenomenon of overthinking. To introduce structured reasoning capabilities into visual understanding models, we further design a novel AtomThink framework with four key modules, including (i) a data engine to generate high-quality multimodal reasoning paths; (ii) a supervised fine-tuning process with serialized inference data; (iii) a policy-guided multi-turn inference method; and (iv) an atomic capability metric to evaluate the single step utilization rate. We conduct extensive experiments to show that the proposed AtomThink significantly improves the performance of baseline MLLMs, achieving more than 10\% average accuracy gains on MathVista and MathVerse. Compared to state-of-the-art structured CoT approaches, our method not only achieves higher accuracy but also improves data utilization by 5 times and boosts inference efficiency by 85.3\%. Our code is now public available in https://github.com/Quinn777/AtomThink.

==> sec/4_exp_old.tex <==
\section{Experiment}
\label{sec:exp}

\begin{figure*}[t]
    \centering
    \includegraphics[width=\textwidth]{img/case_study.pdf} 
    \caption{A case study of AtomThink CoT and GPT-4o generated CoT. Red and green characters denote incorrect and correct responses, respectively. Our model exhibits fewer hallucinations and stronger reasoning abilities as it focuses on the quality of atomic steps. Moreover, our model automatically decomposes the reasoning process semantically, leading to improved readability.}
    \label{fig:case}
\end{figure*}

\subsection{Setup}
\paragraph{Baselines.} Our experiments utilize two open-source MLLMs, including LLaVA-Llama3-8B~\cite{liu2024visual} and EMOVA-8B~\cite{chen2024emova}. We fine-tune only the parameters of their language models and projectors with learning rates of 2e-5 and 2e-6, respectively, and a batch size of 128. We select nine cutting-edge MLLMs for comparison, including OpenAI’s o1~\cite{openai2024_o1}, 4o~\cite{openai2024_4o}, and 4v~\cite{openai2024_4v}, as well as LLava-NeXT-34B~\cite{liu2024llavanext}, InternLM-XComposer2~\cite{zhang2024mavis}, Qwen-VL-Plus~\cite{bai2023qwen}, LLaVA-7B~\cite{liu2024visual}, G-LLaVA-7B~\cite{gao2023gllava}, and MAVIS-7B~\cite{zhang2024mavis}.

\paragraph{Datasets.}
For \textbf{LLaVA-Llama3-8B}, we use LLaVA-665k~\cite{liu2024visual} for supervised fine-tuning (SFT) as a baseline. Additionally, in \textbf{LLaVA w/. Formatted} and \textbf{EMOVA w/. Formatted}, we transfer the source data of AtomMATH into an aligned CoT format for incremental training, ensuring a fair comparison without introducing bells and whistles. For EMOVA-8B, we downsampled its publicly available SFT data~\cite{chen2024emova} to obtain a basic post-training dataset containing about 200k samples. For models with AtomThink, the AMATH-SFT dataset introduced in Section \ref{sec:engine}, is incorporated to introduce atomic reasoning capabilities.

\paragraph{Evaluation Setting.}
We evaluated the performance of our method on MathVista~\cite{lu2023mathvista}, a publicly available benchmark encompassing both general-targeted and mathematics-targeted domains. Additionally, to assess the model's ability to interpret mathematical graphs, we use a more challenging multimodal benchmark, MathVerse~\cite{zhang2025mathverse} for further evaluation. It contains five categories including Text Lite (TL), Text Dominant (TD), Vision Intensive (VI), Vision Dominant (VD), Vision Only (VO).

Out evaluations include four inference settings, including \textbf{Direct}, \textbf{CoT}, \textbf{Quick Think}, and \textbf{Slow Think}. In the \textbf{Direct} setting, we prompt the model to generate a concise final answer. In \textbf{CoT}, the model is instructed to answer the question through step-by-step reasoning. For the \textit{Direct} and \textbf{CoT} evaluations, we use prompts from {lmms-eval} \cite{zhang2024lmmsevalrealitycheckevaluation,lmms_eval2024}. Our AtomThink-models support two additional settings: \textbf{Quick Think} and \textbf{Slow Think}. In \textbf{Quick Think}, our models follow a single, atomic reasoning path based purely on their learned policies, without employing any supplementary search strategies. In \textbf{Slow Think}, enhanced by the PRM, we utilize beam search with beam width of 2 and temperature of 1.0, encouraging our models to engage in more extensive reasoning.

% For both Direct and CoT inference, we follow the instruction provided by \textbf{lmms-eval}~\cite{zhang2024lmmsevalrealitycheckevaluation,lmms_eval2024} to enable model to output answers in specified format. In Quick Think, model generates a single atomic reasoning path solely based on the learned policy, without employing any additional search strategies. When introducing PRM, we employ step-wise or path-wise search strategies to encourage the model to perform more extensive thinking.



\begin{table*}[h!]
\centering
\begin{tabular}{
    c % Model column width
    c % method
    |
    c % general column width
    c % math column width
    c % total column width
    |
    c % Text Lite column width
    c % Text Dominant column width
    c % Vision Intensive column width
    c % Vision Dominant column width
    c % Vision Only column width
    c % total column width
}
\toprule
& & \multicolumn{3}{c|}{\textbf{MathVista}} & \multicolumn{6}{c}{\textbf{MathVerse}} \\
\midrule
\textbf{Model} & \textbf{Inference} & \textbf{General} & \textbf{Math} & \textbf{Total} & \textbf{TL} & \textbf{TD} & \textbf{VI} & \textbf{VD} & \textbf{VO} & \textbf{Total} \\
\midrule
Random Choice & - &- & - & 17.9 & 12.4 & 12.4 & 12.4 & 12.4 & 12.4 & 12.4 \\
Human & - &- &- & -& 70.9 & 71.2 & 61.4 & 68.3 & 66.7 & 66.7 \\
OpenAI o1 & Slow Think* &- & -& 73.9 &- & -&- & -&- &- \\
GPT-4o & CoT & - & -& 63.8 &- & -&- &- &- & - \\
GPT-4V & CoT & -&- & 49.9 & 56.6&63.1 &51.4 &50.8 & 50.3& 54.4 \\
LLaVA-NeXT-34B & Direct & -& -& 46.5 & 25.5 & 33.8 & 23.5 & 20.3 & 15.7 & 23.8 \\
\small{InternLM-XComposer2} & Direct &- & -& 57.6 & 17.0 & 22.3 & 15.7 & 16.4 & 11.0 & 16.5 \\
Qwen-VL-Plus & Direct &- &- & 43.3 &11.1 &15.7 & 9.0 & 13.0 & 10.0 & 11.8 \\
LLaVA-1.5-13B & Direct & -&- & 27.6 & 15.2&19.4 &16.8 &15.2 & 11.3& 15.6\\
G-LLaVA-7B & Direct & -& -& 53.4 & 20.7 &20.9 & 17.2& 14.6& 9.4&16.6 \\
MAVIS-7B & Direct & -&- & - & 29.1 &41.4 & 27.4& 24.9& 14.6&27.5 \\
\midrule
LLaVA-Llama3-8B & Direct & 34.1 & 25.6 & 29.5 & 16.0 & 19.3 & 16.4 & 13.1 & 15.0 & 15.9\\
LLaVA w/. Formatted & CoT & 30.2 & 22.9 & 26.3 & 14.3 & 18.4 & 15.7 & 10.0 & 7.7 &13.2 \\
AtomThink-LLaVA & Direct & 34.4 & 27.2 & 30.5 & 16.0 & 19.3 & 16.2 & 13.1 & 15.0 & 15.9\\
AtomThink-LLaVA & Quick Think & \textbf{36.9} & \textbf{37.0} & \textbf{36.6} & \textbf{22.2} & \textbf{26.6} & \textbf{24.1} & \textbf{20.9} & \textbf{17.9} & \textbf{22.4}\\
AtomThink-LLaVA & Slow Think & \textbf{36.5} & \textbf{41.3} & \textbf{39.1} & \textbf{36.1} & \textbf{42.4} &\textbf{30.0}  &\textbf{36.8}  & \textbf{28.6 }&\textbf{34.7} \\
\midrule
% EMOVA-8B* & Direct & 54.35 & 53.89 & 54.1 & 41 & 42.4 & 33.3 & 42.1 & 9.5 & 31.3 \\
EMOVA-8B-200k & Direct & 52.4 & 51.1 & 51.7 & 34.4 & 39.0 & 33.4 & 30.1 & 23.5 & 32.1 \\
EMOVA w/. Formatted & CoT & 30.9 & 31.3 & 31.1 & 26.5 & 36.5 & 25.3 & 20.4 & 19.8 & 25.7 \\
AtomThink-EMOVA & Direct & 53.9 & 52.4 & 53.1 & 33.6 & 39.0 & 33.8 & 28.0 & 24.4 & 31.8\\
AtomThink-EMOVA & Quick Think & 48.7 & \textbf{54.4} & \textbf{51.8} & \textbf{36.5} & \textbf{42.4} & \textbf{34.1} & \textbf{32.9} & \textbf{29.7} & \textbf{35.1} \\
AtomThink-EMOVA & Slow Think & 48.9 & \textbf{57.0} & \textbf{53.3} &\textbf{42.1}& \textbf{51.5}&\textbf{39.0} &\textbf{36.7} &\textbf{33.1} & \textbf{40.5} \\

\bottomrule
\end{tabular}
\caption{Comparison of accuracy with state-of-the-art methods on MathVista and MathVerse. Our AtomThink LLaVA outperforms the baseline in all sub-tasks across two benchmarks, achieving an average improvement of 14.2\%. Meanwhile, AtomThink EMOVA, with only 8B parameters, surpasses the larger LLaVA-NEXT-34B and even is comparable to GPT-4V.}
\label{tab:main}
\end{table*}




\subsection{Main Results}

\paragraph{Comparison with existing MLLMs.}
In Table~\ref{tab:main}, our AtomThink framework is applied to train LLaVA-Llama3-8B and EMOVA-8B, yielding consistent performance improvements over the original models. When combined with PRM, AtomThink-EMOVA achieves a new state-of-the-art on MathVerse, surpassing GPT-4o and narrowing the gap between MLLMs and human performance. On MathVista, it also achieves performance close to that of GPT-4o. These results demonstrate the framework's strong generalization capability and practical usability.

\paragraph{Quick Think with Intuition.}

Unlike traditional CoT methods, Quick Think generates a stepwise reasoning path through multi-turn conversations, bypassing the need for an additional verifier. This approach offers a computational advantage over Slow Think and highlights the model's intuitive reasoning capabilities. For LLaVA-Llama3-8B, our AtomThink framework surpasses the baseline model, achieving approximately a 10\% improvement on MathVista~\cite{lu2023mathvista} and a 19\% improvement on MathVerse~\cite{zhang2025mathverse}. For AtomThink-EMOVA, Quick Think achieved a score of 38.3\% on MathVerse, outperforming existing open-source MLLMs. These results demonstrate that when a model possesses atomic reasoning capabilities, it can leverage rapid intuition to perform more accurate mathematical reasoning.

\paragraph{LLM Effectively Supervise Visual Reasoning Processes.}

Previous work has shown that process supervision reward models are effective in evaluating intermediate reasoning steps, though these methods have been primarily applied within the domain of language models. We fine-tuned an LLM with A-MATH-PRM and applied it for test-time scaling. As shown in the table, AtomThink-EMOVA, when utilizing PRM with beam search, achieved an additional 2\% improvement on MathVista~\cite{lu2023mathvista} compared to Quick Think. In MathVerse~\cite{zhang2025mathverse}, it even outperformed the closed-source model GPT-4V by 1\%. Additionally, increasing test-time scaling in LLAVA resulted in substantial improvements, positioning it well above its sibling model, LLAVA-1.5-13B.

We find that even when the reasoning process heavily relies on visual dominant inputs, our models can avoid taking incorrect paths by improving text decoding. On the one hand, it is attributed to the AtomThink training process, which encourages MLLM to first understand image before reasoning. On the other hand, it also confirms the effectiveness of test-time extension in multimodal tasks.

\paragraph{Trade-off between General and Math Ability.}
Similar to the conclusions reported in o1, we observe that MLLMs become weaker on general tasks that rely on world knowledge during deep contemplation, demonstrating a trade-off between higher-level reasoning and direct thinking. For instance, LLaVA-Llama3-8B presents a decline in accuracy of 7\% compared to the baseline on the general subset of MathVista, while EMOVA experiences a 17\% reduction. However, after applying PRM-based action search, both models are able to narrow this generalization gap and improve accuracies by 4\% and 16\%, respectively.

\subsection{Atomic Ability Analysis}
We first cluster the reasoning behaviors of GPT-4o into a set of capabilities \(\mathcal{S}\), including Approximation, Verification, Calculation, Variable Definition, Geometric Reasoning, Conclusion Drawing, Graphs Analysis, Equation Formulation, Image Description, Knowledge Introduction, Information Extraction, and Formula Derivation. Using queries in MathVerse~\cite{zhang2025mathverse}, we constructed 500 current states as \(s_i\) with high-quality responses generated by GPT-4o. Subsequently, soft estimations of atomic actions are mapped to \(\mathcal{S}\) for analysis.

% action score analysis
% \noindent\textbf{Ability Analysis.}{\vspace{1.5mm}}
% \vspace{-1.5mm}
\paragraph{Ability Analysis.} Figure \ref{fig:eval} illustrates the distribution of atomic behaviors and capability differences between LLAVA-llama3-8b and EMOVA-8B with their AtomThink-versions. The analysis reveals that AtomThink-Model generally outperforms baseline across most abilities, demonstrating higher scores in areas such as Image Description and Verification. It suggests that our model is capable of more accurate analysis of visual information and demonstrates a degree of self-checking and reflective capability.

\begin{figure}[htbp]
    \centering
    \hspace{-0.5cm}
    \includegraphics[width=0.5\textwidth]{img/model_comparison.pdf} 
    \caption{Comparison to CoT and g1 in MathVista subsets. In contrast to the declining trend observed in g1, AtomThink outperforms the baseline across most subsets.}
    \label{fig:g1}
\end{figure}

\subsection{Comparison with g1}
In Figure \ref{fig:g1}, we compare AtomThink with the state-of-the-art open-source inference strategy, g1\footnote{https://github.com/bklieger-groq/g1}, which employs dynamic prompting to make model focus on single step reflection. In GPT-4o, direct application of g1 for multi-turn reasoning yields a greater improvement over Chain-of-Thought, particularly in numeric and geometric tasks. However, due to the reliance on the inherent reasoning capabilities of large-scale language models, its performance significantly degrades on smaller models such as EMOVA-8B and LLaVA-Llama3-8B. In contrast, our AtomThink framework consistently enhances the performance of these MLLMs.

\subsection{Action Search Ablation}
In Table \ref{tab:search}, we evaluate the impact of direct output, path-wise search and action-wise search strategies on MathVista~\cite{lu2023mathvista} and MathVerse~\cite{zhang2025mathverse} using a subset of 300 samples from each. Results show that even without additional computation, AtomThink-EMOVA's direct prediction accuracy outperforms the original, with improvements of 1.3\%, 1.52\%, and 2.4\%, respectively. The path-wise search method, BoN-Avg, achieves the highest accuracy of 58.68\% on the MathVista~\cite{lu2023mathvista} mathematical tasks, although it experienced a drop on general problems. Meanwhile, both greedy algorithm and beam search show balanced performance across all benchmarks, with the generalization gap between math and general tasks being notably smaller than that of path-wise search.

\begin{table}[ht]
\centering
\resizebox{\columnwidth}{!}{ 
\begin{tabular}{
    l % Left-aligned column for Method
    l % Left-aligned column for Inference
    |
    c % Center-aligned column for MathVista
    c
    c % Center-aligned column for MathVision
    c % Center-aligned column for MathVerse
    c % Center-aligned column for Avg
}
\toprule
\textbf{Model} & \textbf{Method} & \textbf{MathVista-M} & \textbf{MathVista-G} & \textbf{MathVerse} \\
\midrule
EMOVA-200k & Direct & 51.1 & 52.4 & 33.3 & \\
\midrule
\multicolumn{1}{l}{\multirow{2}*{AtomThink}} & Direct & 52.4 & 53.9 & 35.7 & \\
 & Quick Think & 54.2 & 46.7 &38.0 &\\
\midrule
\multicolumn{1}{l}{\multirow{4}*{w/. Path-wise}}  & Majority Voting & 48.8 & 49.4 & 39.0 & \\
 & BoN-Last & 51.2 & 46.8 & 41.3 & \\
 & BoN-Avg & 58.7 & 40.5 & 38.7 \\
 & BoN-Min & 53.7 & 53.2 & 40.0 \\
 \midrule
\multicolumn{1}{l}{\multirow{2}*{w/. Step-wise}} & Greedy & 46.3 & 45.6 & 38.3 & \\
 & Beam Search & 57.1 & 53.2 & 45.3 \\
\bottomrule
\end{tabular}
}
\caption{Ablation study on Path-wise and step-wise search. The results show that both Best-of-N-Min(BoN-Min) and Beam Search exhibit consistent performance improvements.}
\label{tab:search}
\end{table}

\textbf{Limitation}. Due to the limitations in computing infrastructure, we are unable to validate our method on larger MLLMs. Additionally, despite undergoing small-scale manual review, our dataset still lacks step-level golden answers, which may introduce noise into training.






==> sec/5_limitation.tex <==
\section{Limitation}

\begin{Limitation}
Due to the limitations in computing infrastructure, we are unable to validate the boundaries of our method on larger MLLMs. Additionally, despite undergoing small-scale manual review, our Atom-MATH dataset still lacks step-level golden answers, which may introduce noise into training.

\end{Limitation}
